The Symmetrized Holographic Entropy Cone

The holographic entropy cone (HEC) characterizes the entanglement structure of quantum states which admit geometric bulk duals in holography. Due to its intrinsic complexity, to date it has only been possible to completely characterize the HEC for at most $n=5$ numbers of parties. For larger $n$, our knowledge of the HEC falls short of incomplete: almost nothing is known about its extremal elements. Here, we introduce a symmetrization procedure that projects the HEC onto a natural lower dimensional subspace. Upon symmetrization, we are able to deduce properties that its extremal structure exhibits for general $n$. Further, by applying this symmetrization to the quantum entropy cone, we are able to quantify the typicality of holographic entropies, which we find to be exponentially rare quantum entropies in the number of parties.

==> editionlegend.tex <==

\hspace{0pt}\vfill
\noindent\rule{\textwidth}{1pt}



{\vspace{10pt}

Commenting:\vspace{6pt}

\centering
\begin{tabular}{|c|c|}
    \hline
    Author & Command \\\hline
    Matteo Fadel & \textbackslash MF\{comment\} $=$ \MF{comment}\\
    Sergio Hern\'andez-Cuenca & \textbackslash SHC\{comment\} $=$ \SHC{comment} \\
    Max Rota & \textbackslash MR\{comment\} $=$ \MR{comment} \\\hline
\end{tabular}\\

\vspace{10pt}}

{\vspace{10pt}

Editing:\vspace{6pt}

\centering
\begin{tabular}{|c|c|}
    \hline
    Input & Output \\\hline
    \textbackslash soutto\{crossed text\}\{new text\} & \soutto{crossed text}{new text} \\
    \textbackslash goneto\{gone text\}\{new text\} & \goneto{gone text}{new text} \\
    \textbackslash ignore\{ignored text\} & \ignore{commented-out text} \\\hline
\end{tabular}\\

\vspace{10pt}}

{\vspace{10pt}

Writing:\vspace{6pt}

\centering
\begin{tabular}{|c|c|}
    \hline
    Purpose & Implementation \\\hline
    Show labels in margin & Uncomment \emph{\textbackslash usepackage\{showkeys\}} in \emph{setup.sty}\\
    Show labels and in-line refs & Uncomment \emph{\textbackslash usepackage\{showlabels\}} in \emph{setup.sty}\\\hline
\end{tabular}\\

\vspace{10pt}}

\noindent\rule{\textwidth}{1pt}
\vfill

\thispagestyle{empty}
\newpage
